LMAC-TD: Producing Time Domain Explanations for Audio Classifiers

Neural networks are typically black-boxes that remain opaque with regards to their decision mechanisms. Several works in the literature have proposed post-hoc explanation methods to alleviate this issue. This paper proposes LMAC-TD, a post-hoc explanation method that trains a decoder to produce explanations directly in the time domain. This methodology builds upon the foundation of L-MAC, Listenable Maps for Audio Classifiers, a method that produces faithful and listenable explanations. We incorporate SepFormer, a popular transformer-based time-domain source separation architecture. We show through a user study that LMAC-TD significantly improves the audio quality of the produced explanations while not sacrificing from faithfulness.

==> exp_bkp.tex <==
% First of all, in order to establish that the explanations produced by LMAC-TD indeed follow the classifier, we use several different quantitative metrics. We adopt the evaluation metrics employed in the original LMAC paper \cite{paissan24lmac}. The metrics we use are Average Increase (AI) that measures the increase in confidence for the masked-in portion of the interpretation, Average Decrease (AD) that measures how much confidence is lost when the input image is masked, Average Gain (AG) that also measures how much confidence is gained
% after masking the input image. Beyond these metrics we use the Faithfulness (FF) metric defined in the L2I paper \cite{l2i}, and the input Fidelity metric defined in the PIQ paper \cite{paissan2023posthoc}. We also use the Sparseness (SPS) \cite{chalasani2020concise}, and Complexity (COMP) \cite{bhatt2020evaluating} to evaluate the conciseness of the explanations. 

Experimentally, we conduct two sets of experiments, where we evaluate the faithfulness of the produced explanations on In-Domain (ID), and Out-of-Domain (OOD) data. For all experiments, we use a CNN14 classifier \cite{kong2020panns} pretrained on the VGGSound dataset \cite{Chen2020vggsound}. This classifier is later finetuned on the ESC50 dataset \cite{piczak2015dataset} using WHAM! noise \cite{Wichern2019WHAM} augmentation. LMAC-TD is later trained also on the ESC50 dataset with WHAM! noise augmentation. We used series of convtranspose layers for the UNet decoder, to transform the last 4 latent representations of the classifier into the same shape as the encoder output $H_e$. Our implementation can be found through our implementation\footnote{\url{}} with SpeechBrain 1.0 \cite{}.

We compare the faithfulness and complexity numbers obtained through LMAC-TD with several other saliency based methods in the litterature. Namely we compared with several gradient-based methods such as standard saliency maps \cite{simonyan2014deep}, SmoothGrad \cite{smilkov2017smoothgrad}, IntegratedGradients \cite{sundararajan2017axiomatic}, GuidedBackProp \cite{springenberg2015striving}, and decoder based audio specific method, Listen-to-Interpret (L2I) \cite{l2i}, and we also include SHAP \cite{lundberg2017unified}. 

In Table \ref{tab:ID-ESC50}, we report the quantitative results obtained for the In-Domain experiment. We observe that except the AD metric LMAC-TD outperforms standard L-MAC. In terms of SPS metric LMAC-TD is also able to outperform the alternatives. 
In Table \ref{tab:OOD-ESC50} we compare the results obtained on audio mixtures created with ESC50 data. We created mixtures where the dominant class is present with 5 dB SNR. We observe that on most metrics.. 

cem: we should talk about OOD stuff here. 

==> intro_bkp.tex <==
Black-box neural networks obtain impressive performance across a wide range of application domains, but their decision mechanisms typically remain opaque. Post-hoc explanation methods aim to alleviate this issue by highlighting the parts of the input that are deemed most influential for the network decisions \cite{Selvaraju_2019 smilkov2017smoothgrad, Chattopadhay_2018}. %\sout{Post-hoc explanation methods do not alter the original network architecture, and therefore constitute an interesting option to produce explanations while not sacrificing performance.}
\fp{Post-hoc interpreters do not alter the original network architecture and operate \textit{post-hoc} on a pre-trained model. That is, we produce interpretations without constraining the network to interpretable designs\cite{l2i, loiseau2022model, zinemanas2021interpretable, 9914699} or training strategies\cite{flint} that can eventually harm performance.}

% In recent years, there has been progress in %the domain of 
% producing listenable explanations. These works include AudioLIME, SLIME \cite{haunschmid2020audiolime, } which proposed preprocessing L2I \cite{l2i}, which proposed to train a decoder to selectively activate an NMF \cite{} dictionary. Later on L-MAC \cite{} simplified the architecture proposed in L2I to perform inference when producing the explanations. 
In recent years, significant progress has been made in generating post-hoc listenable explanations. Notable works include SLIME \cite{DBLP:conf/ismir/MishraSD17} and AudioLIME \cite{haunschmid2020audiolime}.
SLIME\cite{DBLP:conf/ismir/MishraSD17} segments the spectrogram into time-frequency regions similar to LIME's superpixels for images \cite{lime}, and evaluates each region's importance.
AudioLIME \cite{haunschmid2020audiolime} extracts sources from the audio and assigns a saliency score to each. 
L2I \cite{l2i} introduced a decoder to selectively activate an NMF dictionary \fp{based on the relevance of its components to the predicted class}. 
\fp{L-MAC \cite{paissan24lmac} later simplified L2I’s architecture by introducing a custom loss function to maximise the interpretations faithfulness, while removing the need for a pre-trained NMF dictionary. In LMAC-ZS~\cite{paissan2024listenablemapszeroshotaudio}, the authors adapt the loss function to work with zero-shot classifiers.}
% Even though L-MAC was shown to produce more faithful, and better quality explanations when compared to its alternatives, the filtering is done in the magnitude-STFT domain with a basic separation architecture that uses the phase of the input mixture. This was a good step towards establishing the fact that the framework proposed with L-MAC is able to produce faithful explanations that is able to explain the classifier, and which are also understandable. 
L-MAC generates more faithful and higher-quality explanations than its counterparts. However, it operates in the magnitude-STFT domain with a simple separation architecture that retains the input mixture's phase. Skipping the phase estimation step, L-MAC produces explanations that are both faithful to the classifier and easy to understand but can contain artifacts.
% Despite L-MAC's success in generating more faithful and higher-quality explanations than its counterparts, it operates in the magnitude-STFT domain with a simple separation architecture that retains the input mixture's phase. However, this was a key step in proving that L-MAC can produce explanations that are both faithful to the classifier and easy to understand.

% In recent years, deep learning based source separation reached very impressive levels of performance, obtaining Signal-to-Noise ratios that surpass 20dB on the standard benchmarks such as WSJ0-2Mix \cite{} and Libri2Mix \cite{}. One such architecture that remained state-of-the-art is SepFormer \cite{}. In this paper, we propose to incorporate the SepFormer MaskNet to directly create explanations in the time domain. 

In recent years, deep learning-based source separation has achieved remarkable performance, reaching Signal-to-Noise Ratios above 20dB on benchmarks like WSJ0-2Mix \cite{wsj0-2mix} and Libri2Mix \cite{cosentino2020librimix}. Among the state-of-the-art models is SepFormer \cite{sepformer}. In this paper, we propose \fp{enhancing the quality of LMAC's explanations by} incorporating the SepFormer's MaskNet \fp{in the interpreter}. That is, we generate explanations directly in the time domain, bypassing the need for phase recovery required by L-MAC’s magnitude-STFT approach.

% Our experimental results indicate that LMAC-TD, the time domain version of the L-MAC framework, is able to obtain comparable results in terms of the faithfulness metrics established in the original LMAC paper \cite{paissan24lmac}. 
Our experimental results show that the proposed LMAC-TD, the time-domain version of the L-MAC framework, achieves comparable results in terms of the faithfulness metrics established in the original L-MAC paper \cite{paissan24lmac}, while delivering improved audio quality as demonstrated by our user study.
